Understanding and Mitigating Distribution Shifts For Machine Learning Force Fields

Machine Learning Force Fields (MLFFs) are a promising alternative to expensive ab initio quantum mechanical molecular simulations. Given the diversity of chemical spaces that are of interest and the cost of generating new data, it is important to understand how MLFFs generalize beyond their training distributions. In order to characterize and better understand distribution shifts in MLFFs, we conduct diagnostic experiments on chemical datasets, revealing common shifts that pose significant challenges, even for large foundation models trained on extensive data. Based on these observations, we hypothesize that current supervised training methods inadequately regularize MLFFs, resulting in overfitting and learning poor representations of out-of-distribution systems. We then propose two new methods as initial steps for mitigating distribution shifts for MLFFs. Our methods focus on test-time refinement strategies that incur minimal computational cost and do not use expensive ab initio reference labels. The first strategy, based on spectral graph theory, modifies the edges of test graphs to align with graph structures seen during training. Our second strategy improves representations for out-of-distribution systems at test-time by taking gradient steps using an auxiliary objective, such as a cheap physical prior. Our test-time refinement strategies significantly reduce errors on out-of-distribution systems, suggesting that MLFFs are capable of and can move towards modeling diverse chemical spaces, but are not being effectively trained to do so. Our experiments establish clear benchmarks for evaluating the generalization capabilities of the next generation of MLFFs. Our code is available at https://tkreiman.github.io/projects/mlff_distribution_shifts/.

==> paper_arxiv/s1_intro_arxiv.tex <==
\vspace{-8pt}
\section{Introduction}
\label{sec:intro}
\vspace{-5pt}

Understanding the quantum mechanical properties of atomistic systems is crucial for the discovery and development of new molecules and materials. Computational methods like Density Functional Theory (DFT) are essential for studying these systems, but the high computational demands of such methods limit their scalability. Machine Learning Force Fields (MLFFs) have emerged as a promising alternative, learning to predict energies and forces from reference quantum mechanical calculations. MLFFs are faster than traditional \textit{ab initio} methods, and their accuracy is rapidly improving for modeling complex atomistic systems~\citep{Batzner_2022nequip, schutt_schnet_2017, gasteiger_gemnet_2021, batatia_mace_2022}.

Given the computational expense of \textit{ab initio} simulations for all chemical spaces of interest, there has been a push to train larger and more accurate MLFFs, designed to work well across many different systems. Developing models with general representations that accurately capture diverse chemistries has the potential to reduce or even eliminate the need to recollect data and retrain a model for each new system. To determine which systems an MLFF can accurately describe and to assess the reliability of its predictions, it is important to understand how MLFFs generalize beyond their training distributions. This understanding is essential for applying MLFFs to new and diverse chemical spaces, ensuring that they perform well not only on the data they were trained on, but also on unseen, potentially more complex systems.


We conduct an in-depth exploration to identify and understand distribution shifts. On example chemical datasets, we find that many large-scale models struggle with common distribution shifts \citep{kovács2023maceoff23, shoghi2023jmp, liao2024equiformerv2, batatia2024macemp} (see \sref{sec:distribution_shifts}). These generalization challenges suggest that current supervised training methods for MLFFs overfit to training distributions and do not enable MLFFs to generalize accurately.  
We demonstrate that there are multiple reasons that this is the case, including challenges associated with poorly-connected graphs and learning unregularized representations, evidenced by jagged predicted potential energy surfaces for out-of-distribution systems.    

Building on our observations, we take initial steps to mitigate distribution shifts for MLFFs \update{without test set reference labels} by proposing two approaches: test-time radius refinement and test-time training \citep{sun2020testtime, gandelsman2022testtime, jang2023testtime}. For test-time radius refinement, we modify the construction of test-graphs to match the training Laplacian spectrum, overcoming differences between training and testing graph structures. 
For test-time training (TTT), we address distribution shifts by taking gradient steps on an auxiliary objective at test time. \update{Analogous to self-supervised objectives in computer vision TTT works \citep{gandelsman2022testtime, sun2020testtime, hardt2024test}, we use an efficient prior as a target to improve representations at test time.}

Although completely closing the out-of-distribution to in-distribution gap remains a challenging open machine learning problem \citep{sun2020testtime, gandelsman2022testtime}, our extensive experiments show that our test-time refinement strategies are effective in mitigating distribution shifts for MLFFs. Our experiments demonstrate that low quality data can be used to improve generalization for MLFFs, and they establish clear benchmarks that highlight ambitious but important generalization goals for the next generation of MLFFs.

\update{We summarize our main contributions here:}
\update{
\vspace{-8pt}
\begin{enumerate}
\itemsep-1pt 
    \item We run diagnostic experiments on different chemical datasets to characterize and understand common distribution shifts for MLFFs in \sref{sec:distribution_shifts}.
    \item Based on (1), we take first steps at mitigating MLFF distribution shifts in \sref{sec:methods} with two test-time refinement strategies. 
    \item The success of these methods, validated through extensive experiments in \sref{sec:experiments}, suggests that MLFFs are not being adequately trained to generalize, despite current models having the expressivity to close the gap on the distribution shifts explored in \sref{sec:distribution_shifts}.  
\end{enumerate}}





==> paper_arxiv/s2_distribution_shifts_arxiv.tex <==
\vspace{-5pt}
\section{Distribution Shifts for Machine Learning Force Fields} 
\label{sec:distribution_shifts}



\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{images/distribution_shifts.drawio.png}
    \caption{\textbf{Distribution Shifts for MLFFs.} We visualize distribution shifts based on changes in features, labels, and graph structure.  Typical training samples from SPICE~\cite{Eastman2023spice} and new systems from SPICEv2 \citep{eastman2024spice2} are displayed. An atomic feature shift is illustrated by comparing a three-atom molecule with a larger molecular system containing 91 atoms (left). A force norm shift is shown by the close proximity of an $H_2$ molecule (circled in pink), leading to high force norms \update{(middle)}. A connectivity shift is shown by the tetrahedral geometry in $P_4S_6$, which differs from the typical planar geometry seen during training (right).}  
    \label{fig:dist_shifts}
\vspace{-12pt}
\end{figure*}

\subsection{Problem Setup and Background}
\label{sec:problem_setup}

MLFFs approximate molecule-level energies and atom-wise forces for a chemical structure by learning neural network parameters from data. For a given a molecular structure, the input to the ML model consists of two vectors: $\mathbf{r} \in \R^{n \times 3}$, $\mathbf{z} \in \R^{n \times d}$, where $n$ represents the number of atoms in the molecule, $\mathbf{r}$ are the atomic positions, and $\mathbf{z}$ are the features of the atom, such as atomic numbers or whether an atom is fixed or not. The model outputs $\hat{E} \in \R, \mathbf{\hat{F}} \in \R^{n \times 3}$, which are the predicted total potential energy of the molecule and the predicted forces acting on each atom.
The learning objective is typically formulated as a supervised loss function, which  measures the discrepancy between the predicted energies and forces and reference energies and forces:
\begin{equation}
    \label{eqn:supervised_loss}
    \vspace{-6pt}
    \mathcal{L}(\mathbf{F}, E) =  \lambda_{E} ||E_{ref} - \hat{E}||_2^2 + \lambda_{F} \sum_{i=1}^n ||\mathbf{F_{i, ref}} - \mathbf{\hat{F}_i}||_2^2,
\vspace{-6pt}
\end{equation}
where $\lambda_E, \lambda_F$ are hyperparameters.

Most modern MLFFs are implemented as graph neural networks (GNNs)~\cite{gilmer2017neural}. 
Consequently, $\hat{E}$ and $\mathbf{\hat{F}}$ are functions of $\mathbf{z}$, $\mathbf{r}$, and $A \in \R^{n \times n}$, the adjacency matrix representing the molecule: 
\begin{equation}
    \label{eqn: gnn}
    \hat{E}, \mathbf{\hat{F}} = f(\mathbf{z}, \mathbf{r}, A)
\end{equation}
The atoms in the molecule are modeled as nodes in a graph, and edges are specified by the adjacency matrix that includes connections to all atoms within a specified radius cutoff~\citep{gasteiger_gemnet_2021, batatia_mace_2022}. The adjacency matrix fully determines a graph structure, and thus defines the graph over which the GNN performs its computation.


\subsection{Criteria for Identifying Distribution Shifts}
\label{sec:criteria_ds}

In this section, we formalize criteria for identifying distribution shifts based on the features, labels, and graph structures in chemical datasets. We define these distribution shifts broadly to encompass the diversity of chemical spaces. We also note that distribution shifts can occur independently along each dimension: e.g., a shift in features does not necessarily imply a shift in labels (see \sref{apx:distribution_shifts} for details). This categorization provides a framework for understanding the types of distribution shifts an MLFF may encounter (see \fref{fig:dist_shifts}). \update{This understanding motivates the refinement strategies described in \sref{sec:methods} that take first steps at mitigating these shifts, providing insights into why MLFFs are susceptible to these shifts in the first place.}

\begin{figure}
    
\centering
\includegraphics[width=0.9\linewidth]{images/foundation_bad_large_text.png}
\captionof{figure}{\textbf{Distribution Shifts for Large Models.} We study distribution shifts on four of the largest open-source MLFFs designed for broad chemical spaces. (a) We evaluate MACE-MP on the MPTrj train set. (b) We evaluate MACE-OFF on 10k new molecules from SPICEv2. \update{(c) We evaluate EquiformerV2 on the OC20 out-of-distribution validation set. (d) We evaluate JMP on the ANI-1x test set.} A molecule is considered out-of-distribution if it is more than 1 standard deviation away from the mean training force norm, system size, or connectivity (with respect to the spectral distance defined above \sref{sec:criteria_ds}). Despite their scale, these large foundation models have $2-10\times$ larger force mean absolute errors (MAE) when encountering distribution shifts.}
\label{fig:foundation_bad}
\end{figure}
 
\paragraph{Distribution Shifts in Atomic Features ($\mathbf{z}$).} 
Distribution shifts in atomic features refer to any change in the atomic composition of a chemical system. This includes, but is not limited to, cases where models are trained on systems containing mixtures of organic elements but tested on structures composed solely of carbon, or cases where there is a shift in system size between training and testing. \fref{fig:dist_shifts} illustrates an atomic feature distribution shift by comparing a small carbon dioxide molecule to larger molecular system containing 91 atoms. 

%Distribution shifts in atomic features $\mathbf{z}$ are the most apparent and detrimental to the performance of current state-of-the-art models (see \sref{sec:experiments}). This may involve encountering a molecule with a new element at test time that was not present during training. For example, a model trained on $CO_2$ might be tested on $SiO_2$ without having seen $Si$ during training (see \fref{fig:dist_shifts}). Although this might initially seem like an unreasonably hard task, we argue that a truly general machine learning model for quantum chemistry should be capable of handling arbitrary elements and charges.

\vspace{-8pt}
\paragraph{Distribution Shifts in Forces ($\mathbf{F}$).}
An MLFF may also encounter a distribution shift in the force labels it predicts. A model trained on structures close to equilibrium, with low force magnitudes, might be tested on a structure with higher force norms. \fref{fig:dist_shifts} shows an example of a tightly clustered $H_2$ molecule, which leads to a force norm distribution shift. 


\vspace{-8pt}
\paragraph{Distribution Shifts in Graph Structure and Connectivity ($A$).} Since many MLFFs are implemented as GNNs, they may encounter distribution shifts in the graph structure defined by $A$. We refer to these as connectivity distribution shifts because $A$ determines the graph connectivity used by the GNN. Connectivity distribution shifts are particularly common in molecular datasets, where one could encounter a benzene ring at test time, despite only having trained on long acyclic structures. \fref{fig:dist_shifts} provides an example of a connectivity distribution shift, going from planar training structures to a tetrahedral geometry at test time. 

We identify connectivity distribution shifts by analyzing the eigenvalue spectra of the normalized graph Laplacian:
\begin{equation}
    \label{eqn: graph_laplacian}
    L = I - (D)^{-\frac{1}{2}}A(D)^{-\frac{1}{2}},
\end{equation}
where $D \in \R^{n \times n}$ is the degree matrix ($D_{ii} = \text{degree}(\text{node}_i)$ and $D_{ij} = 0$ for $i \neq j$, $A_{ij} = 1$ if $||r_i - r_j||_2 \leq r_{cutoff}$ and $0$ otherwise), and $I$ is the identity. $L$ has eigenvalues $\lambda_0, \leq \lambda_1, \leq \dots \leq \lambda_{n-1}$, where $\lambda_i \in [0, 2] \; \forall i$, and the multiplicity of the $0$ eigenvalue equals the number of connected components in the graph.

Following previous work \citep{Chung1996_spectral_graph_theory, WILSON_spectral_norm}, we can compare structural differences between graphs by using the spectral distance \citep{Jovanovi2012_spectral_dist}. Since Laplacian spectra are theoretically linked to information propagation in GNNs \citep{WILSON_spectral_norm, digiovanni2023oversquashingmessagepassingneural}, the spectral distance is a natural choice for comparing molecular graphs (see \sref{sec: ttrr} and \sref{apx:theory_rr} for more details).     

\vspace{-8pt}
\paragraph{Observed Distribution Shifts for Large Models.} We contextualize the aforementioned distribution shifts by considering four large models: MACE-OFF, MACE-MP, EquiformerV2, and JMP \citep{kovács2023maceoff23, shoghi2023jmp, liao2024equiformerv2, batatia2024macemp} MACE-OFF is a 4.7M biomolecules foundation model trained on 951k structures primarily from the SPICE dataset \citep{Eastman2023spice}. The 15M parameter MACE-MP foundation model is trained on 1.5M structures from the Materials Project \citep{dengmptrj}. EquiformerV2 is a 150M parameter model trained on 100M+ structures from OC20 \citep{Chanussot_2021_oc20}. The JMP model has 240M parameters and is trained on 100M+ structures from OC20, OC22, ANI-1x, and Transition-1x \citep{Chanussot_2021_oc20, Tran_2023_oc22, Smith2020_ani1x, schreiner2022transition1x}. These models represent four of the largest open-source MLFFs to date, and they have been trained on some of the most extensive datasets available. We focus on these models since their scale is designed for tackling broad chemical spaces.

We examine the generalization ability of MACE-OFF by testing it on 10k new molecules from the SPICEv2 dataset \citep{eastman2024spice2} not included in the MACE-OFF training set. A molecule is defined as out-of-distribution if it is more than 1 standard deviation away from the mean training data force norm, system size, or connectivity (with respect to the spectral distance defined above \sref{sec:criteria_ds}). Despite its scale, MACE-OFF performs worse by an order of magnitude on out-of-distribution systems (see \fref{fig:foundation_bad}a). \update{We also evaluate JMP on the ANI-1x \citep{Smith2020_ani1x} test set defined in \citet{shoghi2023jmp}. JMP also suffers predictably from force norm, connectivity, and atomic feature distribution shifts (see \fref{fig:foundation_bad}d).}

We focus on force norm distribution shifts for MACE-MP and EquiformerV2, since connectivity is more uniform across bulk materials and catalysts, where atoms are packed tightly into a periodic cell. For MACE-MP, we evaluate its performance directly on the entire MPTrj dataset. This model does not have a clear validation set, as it was trained on all of the data to maximize performance \citep{batatia2024macemp}. MACE-MP still clearly performs worse as force norms deviate from the majority of the training distribution (see \fref{fig:foundation_bad}b). The performance deterioration would be more severe with a held-out test set. \update{EquiformerV2 also struggles with high force norm structures when evaluated on the validation out-of-distribution set from OC20 \citep{Chanussot_2021_oc20} (see \fref{fig:foundation_bad}c).}             

\paragraph{Observations.}  
Training larger models with more data is one approach to address these distribution shifts (for example, with active learning \citep{Vandermause2020activelearning, Kulichenko2024}). However, doing so can be computationally expensive. Our diagnostic experiments also indicate that scale alone might not fully address distribution shifts, as naively adding more in-distribution data does not help large models generalize better (see \fref{fig:foundation_bad}). The diversity of chemical spaces makes it exceedingly difficult to know the exact systems that an MLFF will be tested on \textit{a priori}, making it challenging to curate the perfect training set. These observations lead us to develop strategies that mitigate distribution shifts by modifying the training and testing procedure of MLFFs. Importantly, these refinement strategies can be combined with any further architecture and data advances. 

==> paper_arxiv/s3_methods_arxiv.tex <==
\vspace{-5pt}
\section{Mitigating Distribution Shifts with Test-Time Refinement Strategies for Machine Learning Force Fields} 
\label{sec:methods}

Based on the generalization challenges for foundation models (see \sref{sec:distribution_shifts}), we hypothesize that many MLFFs are severely overfitting to the training data, resulting in a failure to learn generalizable representations. Building on our observations in~\sref{sec:distribution_shifts} and to test this hypothesis, we develop two test-time refinement strategies that also mitigate distribution shifts. \update{We focus on test time evaluations, i.e., with access to test molecular structures but without access to reference labels.} First, by studying the graph Laplacian spectrum, we investigate how MLFFs, and GNNs in general \citep{bechlerspeicher2024gnnregular}, tend to overfit to the regular and well-connected training graphs. In \sref{sec: ttrr}, we address connectivity distribution shifts by aligning the Laplacian eigenvalues of a test structure with the connectivities of the training distribution. Second, we show that MLFFs are inadequately regularized, resulting in poor representations of out-of-distribution systems. We incorporate inductive biases from a cheap physical prior using our pre-training and test-time training procedure (\sref{sec: ttt}) to regularize the model and learn more general representations, evidenced by smoother predicted potential energy surfaces. The effectiveness of these test-time refinement strategies, validated through extensive experiments in \sref{sec:experiments} and \sref{apx:more_ttt}, may indicate that MLFFs are currently poorly regularized and overfit to graph structures seen during training, hindering broader generalization.


\vspace{-10pt}
\subsection{Test-Time Radius Refinement}
\label{sec: ttrr}


\FloatBarrier
\noindent
\begin{minipage}{0.42\textwidth}
  We hypothesize that MLFFs tend to overfit to the specific graph structures encountered during training. We can characterize graph structures by studying the Laplacian spectrum of a graph. At test time, we can then identify when an MLFF encounters a graph with a Laplacian eigenvalue distribution that significantly differs from the training graphs (see \ref{sec:criteria_ds}). To address this shift, we propose updating the test graph to more closely resemble the training graphs, thereby mitigating connectivity distribution shifts. Since the adjacency matrix $A$ and graph Laplacian $L$ are typically generated by a radius graph, we refine the radius cutoff at test time. Instead of using a fixed radius cutoff $r_{\text{train}}$ for both training and testing, adjusting the radius cutoff at test time can help achieve a connectivity that more closely resembles the training graphs. 
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.57\textwidth}

\centering
  \includegraphics[width=\linewidth]{images/radius_refinement_2.png}
  \captionof{figure}{\textbf{Test-Time Radius Refinement.} MLFFs tend to overfit to the well-connected graphs seen during training, which can be identified by the clustering of Laplacian eigenvalues around 1. To mitigate connectivity distribution shifts at test time, we find the optimal radius cutoff, which aligns the Laplacian eigenvalues of test graphs with those of the training distribution.}
  \label{fig:tt_rr}
 
\end{minipage}



Formally, for each test structure $j$, we search over $k$ new radius cutoffs $[r_i]_{i=1}^{k}$, calculate the new eigenvalue spectra for $L^{(j)}$ induced by the new cutoff $r_i$, and select the $r_i$ that minimizes the difference between the eigenvalue spectra of the new graph and the training graphs (see \fref{fig:tt_rr}): 
\begin{equation}
\label{eqn:rr}
    r^{(j)}_{\text{test}} = \argmin_{[r_i]_{i=1}^k} D(\lambda_{\text{train}}, \lambda(L^{(j)}(r_i))),
\end{equation}
where $\lambda_{\text{train}}$ is the training distribution of eigenvalues, $\lambda(L^{(j)}(r_i))$ is the Laplacian spectrum for sample $j$ generated with radius cutoff $r_i$, and $D$ is some distance function. We choose the squared spectral distance:
\begin{equation}
    \label{eqn:spectral_distance}
    D(\lambda_{\text{train}}, \lambda(L^{(j)}(r_i))) = \sum_k (\Bar{\lambda}_k - \lambda(L^{(j)}(r_i))_k)^2,
\end{equation}
where, following previous work, $\Bar{\lambda}$ is the average Laplacian spectrum of the training distribution with spectra padded with zeros to accomodate different sized graphs \citep{Chung1996_spectral_graph_theory, Jovanovi2012_spectral_dist}. While averaging the training distribution provides a lossy representation of the training connectivities, it is computationally impractical to compare each new test structure to all training graphs individually. One alternative is to count the number of training graphs within a certain cutoff of the spectral distance to assess how far a test graph is from the training distribution. However, this measure is highly correlated with the simpler spectral distance metric,~\eref{eqn:spectral_distance} (see \fref{fig:sn_vs_count}). Consequently, while per-sample comparisons could be useful in some cases, we use the more computationally efficient spectral distance metric, \eref{eqn:spectral_distance}, in our experiments. For further details and theoretical motivation, see \sref{apx:ttt_details} and \sref{apx:theory_rr}.

Our experiments show that this procedure virtually never deteriorates performance, as one can always revert to the same radius cutoff used during training (see \sref{sec:experiments}). Additionally, we emphasize that we update the envelope function with the new radius to ensure smoothness of the potential energy surface. We verify that this does maintain energy conservation in \tref{tab:nve_rr}. This refinement method addresses the source of connectivity distribution shifts and serves as an efficient and effective strategy for handling new connectivities.   

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.6\linewidth}
         \centering
         \includegraphics[width=\textwidth]{images/ttt_compressed.png}
         \caption{Test-Time Training (TTT)}
         \label{fig:ttt_compressed}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[height=200pt]{images/sali_pes_vertical_sansserif.png}
         \caption{Predicted Potential Energy Surface}
         \label{fig:sali_pes}
    \end{subfigure}
    \caption{\textbf{Test-Time Training Mitigates Distribution Shifts and Smooths Predicted Potential Energy Surfaces.} We hypothesize that due to overfitting, the predicted potential energy surfaces are jagged for out-of-distribution systems. Our proposed test-time training method (TTT, a) regularizes MLFFs by incorporating inductive biases into the model using a cheap prior. Test-time training first learns useful representations from the prior using either joint-training or a pre-train, freeze, and fine-tune approach. TTT then updates the representations at test-time using the prior to improve performance on out-of-distribution samples. We plot the predicted potential energy surface from a GemNet-dT model along the 2 principal components of the Hessian for salicylic acid, a molecule not seen during training, before and after test-time training (b). TTT effectively smooths the potential energy landscape and improves errors.}
    \label{fig:ttt_pes}
    \vspace{-8pt}
\end{figure*}


\vspace{-10pt}
\subsection{Test-Time Training using Cheap Priors}
\label{sec: ttt}
\vspace{-4pt}


We further hypothesize that the current supervised training procedure for MLFFs can lead to overfitting, leading to poor representations for out-of-distribution systems and jagged potential energy landscape predictions (see \fref{fig:sali_pes} for an example on salicylic acid). To address this, we propose introducing inductive biases through improved training and inference strategies to smooth the predicted energy surfaces. The smoother energy landscape from the improved training indicates that the model may have learned more robust representations, mitigating force norm, atomic feature, and connectivity distribution shifts.

We represent these inductive biases as cheap priors, such as classical force fields or simple ML models. These priors can evaluate thousands of structures per second using only a CPU, making them computationally efficient for test-time use. First, we describe our pre-training procedure, which ensures the MLFF learns useful representations from the cheap prior. By leveraging these representations, we can smooth the predicted energy landscape and mitigate distribution shifts by taking gradient steps with our test-time training (TTT) procedure. 



\vspace{-8pt}
\paragraph{Pre-Training with Cheap Physical Priors.}

We propose a training strategy that first pre-trains on energy and force targets from a cheap prior and then fine-tunes the model on the ground truth quantum mechanical labels. Our loss function for one structure is defined as:
\begin{equation}
    \label{eqn:loss}
    \mathcal{L}(\mathbf{F}^M, E^M, \mathbf{F^P}, E^P) = \mathcal{L}_M + \mathcal{L}_P = \sum_{l \in \{M, P\}} \left( \lambda_{E^{l}} ||E^l - \hat{E}^l||_2^2 + \lambda_{F^l} \sum_{i=1}^n ||\mathbf{F_i^l} - \mathbf{\hat{F}_i^l}||_2^2 \right),
\end{equation}
where $\hat{E}, \hat{\mathbf{F}}$ are the predicted energy and forces, and $M$ and $P$ denote the main and prior task, respectively. During pre-training, gradient steps are initially only taken on the prior objective, corresponding to $\mathcal{L}_P$. For fine-tuning, the representation parameters, $\theta_R$, learnt from the prior are kept frozen, and the main task parameters, $\theta_M$, are updated by training only on the main task loss, $\mathcal{L}_M$. Pre-training and fine-tuning can also be merged and the model can be \textit{jointly trained} on both the cheap prior targets and the expensive DFT targets (see \fref{fig:ttt_compressed}). This corresponds to training on $\mathcal{L}_P + \mathcal{L}_M$. Freezing or joint-training both force the main task head to rely on features learnt from the prior. This approach acts as a form of regularization, resulting in more robust representations. It enables the prior to be used to improve the features extracted from an out-of-distribution sample at test time, improving main task performance. For more details on the necessity of proper pre-training for test-time training, see \sref{apx:ttt_details}.  


\vspace{-6pt}
\paragraph{TTT Implementation Details.} For clarity, let us separate our full model into its three components: $g_{\theta_R}$ (the representation model), $h_{\theta_M}$ (the main task head), and $h_{\theta_P}$ (the prior task head). The representation parameters, $\theta_R$, are learned by minimizing $\mathcal{L}$ during joint training (see \eref{eqn:loss}), or by minimizing $\mathcal{L}_P$ during pre-training and then freezing them during the fine-tuning phase. Test-time training involves the following steps:
\begin{enumerate}
\vspace{-6pt}
    \item \textbf{Updating representation parameters.} At test-time, we update $\theta_R$ by minimizing the prior loss, $\mathcal{L}_P$, on samples from the test distribution $\mathcal{D}_{test}$, which are labeled by the cheap prior. This is expressed as:
\begin{equation}
    \label{eqn:ttt}
    \theta_R^{\prime} = \argmin_{\theta_R} \mathbb{E}_{(\mathbf{r}, \mathbf{z}, \mathbf{F^p}, E^p) \sim \mathcal{D}_{test}} [ \mathcal{L}_P(h_{\theta_P} \circ g_{\theta_R}(\mathbf{r}, \mathbf{z}), \mathbf{F^p}, E^p) ].
\end{equation}
During this process, the prior head parameters, $\theta_P$, are kept frozen during test-time updates. This incorporates inductive biases about the out-of-distribution samples into the model, regularizing the energy landscape and helping the model generalize (see \fref{fig:sali_pes} and \fref{fig: more_pes}).  

\item \textbf{Prediction on test set.} Once the representation parameters are updated, we predict the main task labels for the test set using the newly adjusted representation:
\begin{equation}
    \label{eqn:ttt_pred}
    \hat{E}, \hat{\mathbf{F}} = h_{\theta_M} \circ g_{\theta_R^{\prime}}(\mathbf{r}, \mathbf{z}).
\vspace{-5pt}
\end{equation}
\end{enumerate}
We recalculate the parameters $\theta_R^{\prime}$ with \eref{eqn:ttt} when a new out-of-distribution region is encountered (i.e., when testing on a new system). See \fref{fig:ttt_compressed} for an outline of our method. 

We formalize the intuition behind TTT for MLFFs in the following theorem, where we look at TTT with a simple Lennard-Jones prior \citep{lj}:
\begin{theorem}[] \label{theorem:ttt_mt}
If the reference energy calculations asymptotically go to $\infty$ as pairwise distances go to $0$, then there exist test-time training inputs such that a gradient step on the prior loss, with the Lennard-Jones potential, reduces the main task loss on those inputs. 
%\vspace{-6pt}
\end{theorem}


We prove Theorem \ref{theorem:ttt_mt} by showing that there exist points where the errors on the prior and main task are correlated ($\text{sign}(\hat{E}^P - E^P) = \text{sign}(\hat{E}^M - E^M)$), and that the main task head and the prior task head use similar features ($\theta_P^T \theta_M > 0$). Building off of the theoretical result in \citet{sun2020testtime}, this implies that TTT on these points with prior labels improves main task performance. For a detailed proof, see \sref{apx:theory_rr}.






     



 




==> paper_arxiv/s4_results_arxiv.tex <==
\vspace{-8pt}
\section{Experiments}
\label{sec:experiments}
\vspace{-5pt}

We conduct experiments on chemical datasets to both identify the presence of distribution shifts and evaluate the effectiveness of our test-time refinement strategies to mitigate these shifts. In \sref{exp:spice_maceoff}, we find distribution shifts on the SPICE dataset with the MACE-OFF foundation model \citep{Eastman2023spice, kovács2023maceoff23}. In \sref{exp:sim_md17}, we explore extreme distribution shifts and demonstrate that our test-time refinement strategy enables stable simulations on new molecules, even when trained on a limited dataset of 3 molecules from the MD17 dataset \citep{chmiela_machine_2017}. Finally, in \sref{exp:h2l_md22}, we assess how our test-time refinement strategy can handle high force norms in the MD22 dataset when the model is trained only on low force norms. Although matching in-distribution performance (without access to ground truth labels) remains a challenging open machine learning problem \citep{sun2020testtime, gandelsman2022testtime}, our experiments indicate that test-time refinement strategies are a promising initial step for addressing distribution shifts with MLFFs. The improvements from these test-time refinement strategies also suggest that MLFFs can be trained to learn more general representations that are resilient to distribution shifts. Additional experiments with more models, datasets, and priors are provided in \sref{apx:more_ttt}.      

\vspace{-8pt}
\subsection{Distribution Shifts: Training on SPICE and testing on SPICEv2}
\vspace{-5pt}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/finetuning_data.png}
    \caption{\textbf{Test-Time Training Decreases the Amount of Fine-Tuning Data Needed to Match In-Distribution Performance.} We fine-tune GemNet-T models, trained on SPICE, on new molecules from the SPICEv2 dataset. Applying TTT on the new data before fine-tuning decreases the amount of training data needed to match the in-distribution performance by $10\times$. Applying TTT before fine-tuning also decreases the final error by 25\% when training on all the data.}
    \label{fig:ft_data_spice}
\end{figure}

\label{exp:spice_maceoff}
We investigate distribution shifts from the SPICE dataset to the SPICEv2 dataset \citep{Eastman2023spice, eastman2024spice2} by analyzing the MACE-OFF foundation model \citep{kovács2023maceoff23}. As shown in \fref{fig:spice_force_norms}, \fref{fig:spice_connectivity}, and \fref{fig:spice_new_elements}, we observe that despite being trained on 951k data points and scaled to 4.7M parameters, MACE-OFF experiences force norm, connectivity, and atomic feature distribution shifts when evaluated on 10k new molecules from SPICEv2 \citep{eastman2024spice2}. Any deviation from the training distribution, shown in gray, predictably results in an increase in force error. 

We evaluate the effectiveness of our test-time refinement strategies in mitigating these distribution shifts. For the MACE-OFF model, we implement test-time radius refinement (RR) by searching over 10 different radius cutoffs and selecting the one that best matches the training Laplacian eigenvalue distribution (see \sref{sec: ttrr}). We also train a GemNet-T model on \update{the same} training data used by MACE-OFF, using the pre-training, freezing and fine-tuning method described in \sref{sec: ttt}, with the sGDML model as the prior \citep{Chmiela_2019sgdml}. To show that TTT is prior agnostic, we additionally train a model that uses the semi-empirical GFN2-xTB as the prior \citep{semiempirical}.
See \ref{apx:exp_details} for more details. 

\vspace{-10pt}
\paragraph{Force Norm Distribution Shifts.}
Both MACE-OFF and GemNet-T deteriorate in performance when encountering systems with force norms different from those seen during training, as shown in \fref{fig:spice_force_norms}. Interestingly, this performance drop occurs for both higher and \textit{lower} force norms than those in the training set. Test-time training reduces errors for GemNet-T on out-of-distribution force norms, and also helps decrease errors for the new systems that are closer to the training distribution. The results in \fref{fig:spice_force_norms} specifically filter out atomic feature shifts and different connectivities to isolate the effect of force norm distribution shifts.

\vspace{-10pt}
\paragraph{Connectivity Distribution Shifts.}
For both MACE-OFF and GemNet-T, force errors increase when the connectivity of a test graph differs from that of the training graphs, as measured by the spectral distance (see \eref{eqn:spectral_distance}). Our test-time radius refinement (RR) technique (see \sref{sec: ttrr}) applied to MACE-OFF effectively mitigates connectivity errors at minimal computational cost. Test-time training also effectively mitigates connectivity distribution shifts, as shown in (\fref{fig:spice_connectivity} and \tref{tab: spice_rr_indiviual}). Note that \fref{fig:spice_connectivity} isolates connectivity distribution shifts by filtering out-of-distribution force norms and atomic features. \update{See \sref{apx:ttrr_jmp} for RR results with the JMP model on the ANI-1x dataset.}  

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/force_norm_100p.png}
    \caption{\textbf{Evaluating Distribution Shifts for Force Norms on SPICEv2.} We evaluate MACE-OFF on new molecules from the SPICEv2 dataset with varying force norms. (a) Test structures with different force norms relative to the training distribution (shown in gray) incur larger force errors for MACE-OFF. We also train a GemNet-T model, and then apply test-time training (TTT), mitigating this shift. (b) We highlight the top 10\% of molecules with the greatest improvement to demonstrate that TTT is effective even for structures that are near the training distribution.} 
    \label{fig:spice_force_norms}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/connect_sd.png}
    \caption{\textbf{Evaluating Connectivity Distribution Shifts on SPICEv2.} We evaluate MACE-OFF on new molecules from the SPICEv2 dataset with varying connectivity, defined by the spectral distance to the average training graph (see \sref{sec: ttrr} for details). (a) Test structures with different connectivity relative to the training distribution (shown in gray) incur larger force errors for MACE-OFF. Test-time training (TTT) applied to a GemNet-T model and test-time radius refinement (RR) applied to MACE-OFF are both able to mitigate this performance drop at minimal computational cost. (b) We highlight the top 10\% of molecules with the greatest improvement to demonstrate that TTT is effective even for connectivities close to the training distribution.}
    \label{fig:spice_connectivity}
\vspace{-12pt}
\end{figure}

\vspace{-10pt}
\paragraph{Atomic Feature Distribution Shifts.} MACE-OFF and GemNet-T both perform poorly when encountering molecules with atomic features that differ from their training distributions. In particular, MACE-OFF and GemNet-T struggle with molecules that are both larger and smaller than those seen in training, and with systems that have a different proportion of carbon atoms than seen in training (see \fref{fig:spice_new_elements}). Test-time training reduces errors across both of these atomic feature distribution shifts for GemNet-T. We filter out out-of-distribution connectivities and force norms to isolate the effect of atomic feature distribution shifts. 


%Unsurprisingly, MACE-OFF and GemNet-T perform poorly when they encounter new elements at test time. \fref{fig:spice_new_elements} shows that test-time training can reduce errors on systems with new elements, sometimes by a factor of 10 for specific molecules. While this is a challenging generalization task, we argue that achieving this should be a goal for a true chemistry foundation model, akin to first-principles methods that model the entire periodic table.  Collecting more data for new elements is an option but can be prohibitively expensive, especially for atoms with many electrons. TTT provides a better starting point and reduces the amount of data that needs to be collected (see \fref{fig:ft_after_ttt}).     


\vspace{-12pt}
\paragraph{Aggregated Results and Takeaways.} We present aggregated results on the SPICEv2 distribution shift benchmark, where a model is trained on SPICE and evaluated on 10k new molecules from SPICEv2. The large MACE-OFF foundation model trains on 951k samples but still suffers from distribution shifts on the new structures from SPICEv2. We also see that (1) the RR method mitigates connectivity distribution shifts for MACE-OFF at minimal computational cost (see \tref{tab:agg_spicev2}) and
(2) using TTT with the GemNet-T model performs the best on the new molecules from SPICEv2, highlighting the effectiveness of training strategies for mitigating distribution shifts. Practically, these lower force errors also translate into better MD simulations and improved structure relaxations (see \sref{apx:indvidual_mols_spicev2}). 

\FloatBarrier
\noindent
\begin{minipage}{0.45\textwidth}
  Since the improvements from RR and TTT are right-skewed, meaning many molecules show small improvements while some see large gains, we highlight the 10\% of molecules with the greatest improvement in \fref{fig:spice_force_norms}b, \fref{fig:spice_connectivity}b, and \fref{fig:spice_new_elements}b. We also present results for individual molecules in \tref{tab: spice_ttt_indiviual} and \tref{tab: spice_rr_indiviual} to show that TTT and RR can help across a range of errors. Both TTT and RR improve results on molecules that already have low errors, and bring many molecules with high errors close to the in-distribution performance (\update{see \fref{fig: ttt_rr_chem_acc} which shows that more than $8,000/10,000$ molecules have errors below 25 meV / Å}). 

\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.5\textwidth}
  \setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{cc}
\toprule
    \textbf{Model}                 & \makecell{\textbf{SPICEv2 Test Set} \\ \textbf{Force MAE (meV/Å)}} \\ \hline
MACE-OFF             & $26.75 \pm 0.65$           \\
 +RR (ours)&$26.0 \pm 0.64$            \\ 
GemNet-T             & $22.9 \pm 1.4$             \\ 
+TTT (ours)& $\mathbf{19.9 \pm 1.0}$    \\ \bottomrule
\end{tabular}
\captionof{table}{\textbf{Aggregated Results on SPICEv2 Distribution Shift Benchmark.} 
We provide aggregated results on the SPICEv2 distribution shift benchmark \update{with 95\% confidence intervals}. TTT and RR are both able to effectively mitigate errors across the $10$k unseen molecules from SPICEv2. The relative improvements observed are in line with previous test-time training work \citep{gandelsman2022testtime, sun2020testtime}.}
\label{tab:agg_spicev2}

% \begin{tabular}{ccc}
% \toprule
%                      & \multicolumn{2}{c}{\textbf{SPICEv2 Test Set Force MAE (meV / Å)}} \\
%                      & With New elements           & No New Elements       \\ \hline
% MACE-OFF             & $71.2 \pm 1.3$              & $26.75 \pm 0.65$           \\
%  +RR (ours)& $68.1 \pm 1.6$              &$26.0 \pm 0.64$            \\ 
% GemNet-T             & $64.0 \pm 2.5$              & $22.9 \pm 1.4$             \\ 
% +TTT (ours)& $\mathbf{51.0 \pm 1.8}$     & $\mathbf{19.9 \pm 1.0}$    \\ \bottomrule
% \end{tabular}
% \captionof{table}{\textbf{Aggregated Results on SPICEv2 Distribution Shift Benchmark.} 
% We provide aggregated results on the SPICEv2 distribution shift benchmark \update{with 95\% confidence intervals}. TTT and RR are both able to effectively mitigate errors across the $10$k unseen molecules from SPICEv2.}
% \label{tab:agg_spicev2}

\end{minipage}


The ability of TTT and RR to mitigate distribution shifts supports the hypothesis that MLFFs easily overfit to training distributions, even with large datasets. By improving the connectivity and learning more general representations of test molecules, RR and TTT diagnose the specific ways in which MLFFs overfit. These experiments suggest that improved training strategies could help learn more general models.

\paragraph{Test-Time Training and Fine-Tuning.} While TTT can enable accurate MD simulations for new systems without access to any reference labels (see \sref{exp:sim_md17} and \sref{apx:indvidual_mols_spicev2}), a practitioner may prefer to fine-tune a model on more out-of-distribution data to match the in-distribution performance. We examine how TTT can provide a better starting point for fine-tuning by learning more robust representations for new systems. 

We take the GemNet-T models from the previous section and fine-tune them with varying amounts of structures from the SPICEv2 dataset \citep{eastman2024spice2}. We evaluate how much data is required to match the in-distribution force error on SPICE ($12.9$ meV/Å) when tested on the 10k new molecules from SPICEv2. The vanilla GemNet-T model matches the in-distribution performance when trained on half of the SPICEv2 data. In contrast, using our TTT procedure before fine-tuning allows the model to reach the same performance with only $5\%$ of the data — a $10\times$ reduction. Additionally, TTT reduces the final error by $25\%$ even when fine-tuning on the entire SPICEv2 dataset. See \fref{fig:ft_data_spice} for details.

\vspace{-6pt}
\subsection{Evaluating Generalization with Extreme Distribution Shifts: Simulating Unseen Molecules}
\label{exp:sim_md17}

\begin{figure}
\centering
\begin{subfigure}{0.49\linewidth}
  \centering
  \includegraphics[width=0.95\linewidth]{images/naph_hr.png}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
  \centering
  \includegraphics[width=0.95\linewidth]{images/tolu_hr.png}
\end{subfigure}

\caption{\textbf{Testing Molecular Dynamics Simulations.} TTT enables stable simulations that accurately reconstruct observables, such as the distribution of interatomic distances, for molecules not seen during training (orange). In contrast, predictions without TTT for these unseen molecules result in unstable simulations and inaccurate $h(r)$ curves (blue). Simulations without TTT remained unstable even with a timestep reduced by $5,000\times$.} 
\label{fig:hr}
\end{figure}

We establish an extreme distribution shift benchmark to evaluate the generalization ability of MLFFs on the MD17 dataset \citep{chmiela_machine_2017}. This benchmark is specifically designed to highlight how MLFF training strategies tend to overfit to narrow problem settings, and to evaluate how new training strategies can improve robustness. We train a single GemNet-dT model \citep{gasteiger_gemnet_2021} on $10$k samples each of aspirin, benzene, and uracil. We then evaluate whether this model can simulate two new molecules, naphthalane and toluene, which were unseen during training. Next, we evaluate whether TTT can address the distribution shifts to the new molecules. Using the same procedure outlined in \sref{sec: ttt}, we pre-train on the 3 molecules in the training set with the sGDML prior, then freeze the representation model and fine-tune on the quantum mechanical labels. We then perform TTT before simulating the new molecules (see \sref{sec: ttt}). This is an extremely challenging generalization task for MLFFs due to the limited variety of training molecules. Nevertheless, we believe that a model capable of accurately capturing the underlying quantum mechanical laws should be able to generalize to new molecules.   

We evaluate the stability of simulations over time by measuring deviations in bond length, following \citet{fu2023forces}. We additionally calculate the distribution of interatomic distances $h(r)$, a low dimensional descriptor of 3D molecular structures, to measure the quality of the simulations \citep{Zhang_2018, fu2023forces, raja2025stabilityaware}. See \sref{apx:exp_details} for more details.    

\vspace{-10pt}
\paragraph{Simulation Results.} As shown in \fref{fig:hr}, TTT enables stable simulations of unseen molecules that accurately reproduce the distribution of interatomic distances $h(r)$. Without TTT, the GemNet-dT model trained only on aspirin, benzene, and uracil is unable to stably simulate the new molecules and produces poor $h(r)$ curves. Even when we reduce the timestep by a factor of 5,000, the simulations without TTT remains unstable. \update{We also find that TTT enables stable NVE simulations (see \sref{apx:nve_md17}).} Furthermore, TTT provides a better starting point for fine-tuning, decreasing the amount of data needed to reach the in-distribution performance by more than $20\times$ (see \sref{apx:nve_md17}). Given that GemNet-dT + TTT can produce reasonable simulations without access to quantum mechanical labels of the new molecules, test-time refinement methods could be a promising direction for addressing distribution shifts. 


==> paper_arxiv/s5_conclusion.tex <==
\vspace{-8pt}
\section{Conclusion}

We have demonstrated that state-of-the-art MLFFs, even when trained on large datasets, suffer from predictable performance degradation due to distribution shifts. By identifying shifts in atomic features, force norms, and connectivity, we have developed methods to diagnose the failure modes of MLFFs. Our test-time refinement methods represent initial steps in mitigating these distribution shifts, showing promising results in modeling and simulating systems outside of the training distribution. These results provide insights into how MLFFs overfit, suggesting that while MLFFs are becoming expressive enough to model diverse chemical spaces, they are not being effectively trained to do so. This may indicate that training strategies, alongside data and architecture innovations, will be important in improving MLFFs. Finally, our experiments serve as benchmarks for evaluating the generalization ability of the next generation of MLFFs. 
    


==> paper_arxiv/s6_related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Distribution Shifts.} There is a long line of literature studying distribution shifts in the machine learning community, which we briefly summarize here. \citet{sugiyama07_domainshift} demonstrated how to perform importance weighted cross validation to perform model selection under distribution shifts. Methods have been proposed to measure and improve the robustness of models to distribution shifts in images \citep{taori2020_imgds, zhao2022oodimg} and language \citep{ds_language}. Numerous methods have been proposed to tackle distribution shifts including, but not limited to, techniques based on meta learning \citep{NEURIPS2020_oodmaml} and ensembles \citep{Zhou_2021_dsensemble}.

Recent work has also begun identifying generalization challenges with MLFFs \citep{Li2025_oodmat, Bihani2024_egraff}. \citet{deng2024overcomingsystematicsofteninguniversal} find that MLFFs systematically underpredict energy surfaces, and that this underprediction can be ameliorated with a small number of fine-tuning steps on reference calculations. Our experiments complement these initial findings of underestimation, and we also identify other types of distribution shifts, like connectivity and atomic feature shifts. Our proposed test-time refinement solutions are also able to mitigate distribution shifts \textit{without} any reference data, and they provide insights into \textit{why} MLFFs are unable to generalize.


\paragraph{Multi-Fidelity Machine Learning Force Fields.}

\citet{Behler2007} popularized the use of machine learning for modeling force fields, leading to numerous downstream applications \citep{Artrith2011} and refinements to model increasingly complicated systems \citep{Drautz2019}. More recent work has explored training MLFFs with observables \citep{Fuchs2025_obs, raja2025stabilityaware, Han2025}, distilling MLFFs with physical constraints \citep{amin2025towards}, and using multiple levels of theory during training. \citet{amin2025towards} found that knowledge distillation can enable smaller models to outperform larger models in certain specialized tasks, suggesting that the larger MLFFs may not have been trained in a way that fully leverages their capacity. \citet{Jha2019_transfer}, \citet{Gardner2024_syntheticcarbon}, and \citet{shui2022injecting_domainknowledge} leveraged cheap or synthetic data to improve data efficiency and accuracy. \citet{deltalearning} popularized the $\Delta$-learning approach \citep{Bogojeski2020_delta}, where a model learns to predict the difference between some prior and the reference quantum mechanical targets. Multi-fidelity learning generalizes $\Delta$-learning by building a hierarchy of models that predict increasingly accurate levels of theory \citep{multifidelity_2023,Vinod_2023multifidelity2, Forrester2007_multifidelity, Heinen2024-multifidelity}. Making predictions in the hierarchical multi-fidelity setting corresponds to evaluating a baseline fidelity level and then refining this prediction with models that provide corrections to more accurate levels of theory in the hierarchy. 

Our work differs from these works in several ways. We focus on developing training strategies that address distribution shifts. In contrast to prior multi-fidelity works, we learn \textit{representations} from multiple levels of theory using pre-training, fine-tuning, and joint-training objectives. Rather than fine-tuning all the model weights like in \citet{Jha2019_transfer}, \citet{Gardner2024_syntheticcarbon}, and  \citet{shui2022injecting_domainknowledge}, we explore freezing and regularization techniques that enable test-time training. Our new test-time objectives update the model's representations when faced with out-of-distribution examples, improving performance on out-of-distribution systems. Multi-fidelity approaches by themselves do not tackle the challenge of transferring to new, unseen systems at test-time. Nevertheless, combining our training strategies with other multi-fidelity approaches presents an interesting direction for future work.     

\paragraph{Test-Time Training.}
The test-time training (TTT) framework adapts predictive models to new test distributions by updating the model at test-time with a self-supervised objective \citet{sun2020testtime}. \citet{sun2020testtime} demonstrated that forcing a model to use features learnt from a self-supervised objective during the main task allows the model to adapt to out-of-distribution examples by tuning the self-supervised objective. Follow up work showed the benefits of TTT across computer vision and natural language processing, exploring a range of self-supervised objectives \citep{gandelsman2022testtime, jang2023testtime, hardt2024test}. 




==> paper_arxiv/s8_acknowledgements.tex <==
\section{Acknowledgements}

We thank Sanjeev Raja, Rasmus Lindrup, Yossi Gandelsman, Aayush Singh, Alyosha Efros, Eric Qu, and Yuan Chiang for the thoughtful discussions and feedback on this manuscript. This work was supported by the Toyota Research Institute as part of the Synthesis Advanced Research Challenge. This research used resources of the National Energy Research Scientific Computing Center (NERSC), a U.S. Department of Energy Office of Science User Facility located at Lawrence Berkeley National Laboratory, operated under Contract No. DE-AC02-05CH11231. 

==> paper_arxiv/s9_author_contribution.tex <==
\section{Author Contributions}

\credit{TK}{1,1,1,0,1,1,0,1,1,0,1,1,1,1}
\credit{ASK}{1,0,0,1,1,1,1,1,0,1,1,1,1,1}


\begin{center}
\small\bfseries
\insertcreditsgranular
\end{center}

==> s9_author_contribution.tex <==
\section{Author Contributions}

\credit{TK}{1,1,1,0,1,1,0,1,1,0,1,1,1,1}
\credit{ASK}{1,0,0,1,1,1,1,1,0,1,1,1,1,1}


\begin{center}
\small\bfseries
\insertcreditsgranular
\end{center}
